Human Aligned Compression for Robust Models

Adversarial attacks on image models threaten system robustness by introducing imperceptible perturbations that cause incorrect predictions. We investigate human-aligned learned lossy compression as a defense mechanism, comparing two learned models (HiFiC and ELIC) against traditional JPEG across various quality levels. Our experiments on ImageNet subsets demonstrate that learned compression methods outperform JPEG, particularly for Vision Transformer architectures, by preserving semantically meaningful content while removing adversarial noise. Even in white-box settings where attackers can access the defense, these methods maintain substantial effectiveness. We also show that sequential compression--applying rounds of compression/decompression--significantly enhances defense efficacy while maintaining classification performance. Our findings reveal that human-aligned compression provides an effective, computationally efficient defense that protects the image features most relevant to human and machine understanding. It offers a practical approach to improving model robustness against adversarial threats.

==> sec/0_abstract.tex <==
\begin{abstract}
Adversarial attacks on image classification models pose a significant challenge to the robustness and security of machine learning systems. These attacks subtly manipulate input images, causing misclassification while remaining imperceptible to humans. In this paper, we explore the use of lossy image compression as a defense mechanism against adversarial attacks, especially the effectiveness of learned compression models, which work at very low bitrates. We conduct experiments on two learned compression models, HiFiC and ELIC, and compare them to JPEG compression. We show the trade-off between compression quality and defensive strength by conducting experiments at different levels of compression. We then compute the accuracy for multiple different adversarial attacks on a subset of ImageNet and show that using learned compressions leads to more effective defenses. We also perform attacks in a white-box setting to test the robustness of our defenses against a strong adversary. Additionally, we explore the impact of repeatedly compressing and decompressing in sequence, which we show to increase the effectiveness of a defense.
 
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
In recent years, the field of image classification has witnessed remarkable advancements, largely driven by the development of deep learning models\cite{he2015deepresiduallearningimage} \cite{dosovitskiy2021imageworth16x16words}. These models have achieved state-of-the-art performance in various image recognition tasks, from object detection \cite{NIPS2013_f7cade80} \cite{10028728} to medical imaging \cite{shenmedical2017}. However, their vulnerability to adversarial attacks has emerged as a significant concern, particularly in critical applications such as autonomous driving, healthcare diagnostics, and surveillance systems.

Adversarial attacks\cite{szegedy2014intriguingpropertiesneuralnetworks} involve the deliberate introduction of small perturbations to input images, which are imperceptible to humans but can reliably lead to misclassifications.

To mitigate the impact of adversarial attacks, researchers have explored a variety of defense mechanisms\cite{madry2019deeplearningmodelsresistant}. One promising approach is the use of lossy image compression techniques\cite{dziugaite2016studyeffectjpgcompression}. Lossy image compression, traditionally used to reduce storage and transmission costs by discarding some information, can also lead to the loss of some of the small perturbations introduced by an adversary. Therefore, compressing and then decompressing an image can be used as a defense mechanism to make a model more robust towards adversarial attacks.

This thesis delves into the potential of learned image compressions as a defense against adversarial attacks, comparing them to traditional compression methods, and evaluating their strength against different attacks. We also test the defense strength in a white-box setting, where the adversary has access to the defense and can adapt the attack. Furthermore, we analyze the trade-offs between compression levels and classification accuracy and measure the computational overhead such a defense generates, providing insights into how to optimize this defense strategy for real-world applications.

By exploring the intersection of image compression and adversarial defense, this work aims to contribute to the development of more secure and reliable image classification systems. The findings presented offer insight into the strengths and weaknesses of well-established compression techniques in creating deep learning models which are more resilient against adversarial threats.

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Adversarial attacks}

Adversarial examples have become a critical concern in machine learning, particularly regarding the robustness and security of deep learning models. These examples are carefully crafted inputs designed to mislead models into making incorrect predictions. The phenomenon was first identified by Szegedy \etal \cite{szegedy2014intriguingpropertiesneuralnetworks}, who demonstrated that adding subtle, imperceptible perturbations to images could cause neural networks to misclassify them with high confidence.

Kurakin \etal \cite{kurakin2017adversarialexamplesphysicalworld} extended the study of adversarial attacks to the physical world, showing that printed images with adversarial perturbations could still deceive classifiers when captured through a camera. This work underscored the real-world implications of adversarial attacks beyond purely digital environments.

In response to these challenges, various defense mechanisms have been proposed. Madry \etal \cite{madry2019deeplearningmodelsresistant} introduced adversarial training, a technique in which models are trained on adversarial examples to improve their robustness. Papernot \etal \cite{papernot2016distillationdefenseadversarialperturbations} proposed defensive distillation, leveraging knowledge distillation \cite{hinton2015distillingknowledgeneuralnetwork}—a technique that compresses an ensemble of models into a smaller model—to enhance resistance against adversarial attacks. Another approach involves preprocessing inputs to remove adversarial perturbations before classification, which can be achieved using image compression techniques \cite{dziugaite2016studyeffectjpgcompression}.Despite these efforts, achieving a comprehensive defense against adversarial attacks remains an open problem. 

\subsection{Image compression as adversarial defense}

Previous studies have demonstrated that JPEG compression can enhance model robustness against adversarial attacks. Dziugaite \etal. \cite{dziugaite2016studyeffectjpgcompression} showed that JPEG compression can mitigate the effects of small adversarial perturbations, even when using a relatively high quality parameter of 75. To achieve this, an image suspected of containing adversarial perturbations is first compressed and then decompressed using the JPEG format. The compression and decompression process removes small perturbations introduced by adversarial attacks, thereby reducing their effectiveness.

However, Shin \etal \cite{shin2017jpeg} demonstrated that the defensive effectiveness of JPEG compression can be significantly diminished by leveraging a differentiable approximation of the JPEG algorithm. By propagating gradient information through both the JPEG compression process and the model, adversarial attacks can generate perturbations that persist even after the compression and decompression steps.

\subsection{Learned lossy image compression}

Learned lossy image compression is a technique that utilizes machine learning to achieve efficient image compression. While traditional algorithms such as JPEG struggle to maintain high visual quality at very low bitrates, learned compression techniques can produce significantly clearer images under these conditions \cite{agustsson2019generativeadversarialnetworksextreme}. This increased information loss may, in turn, provide an advantage in defending against adversarial attacks.

HiFiC \cite{mentzer2020highfidelitygenerativeimagecompression} is a learned compression method designed to generate visually appealing reconstructions while preserving information critical to human perception. The model employs an architecture based on Generative Adversarial Networks (GANs). A user study evaluating HiFiC demonstrated that its reconstructions were preferred over those from other methods, even when using half the number of bits per pixel.

ELIC \cite{he2022elicefficientlearnedimage}, which stands for Efficient Learned Image Compression with Unevenly Grouped Space-Channel Contextual Adaptive Coding, is a model optimized for both speed and efficiency in image compression. Experimental results demonstrate that ELIC outperforms previous learned compression methods, like Minnen \etal \cite{minnen2018jointautoregressivehierarchicalpriors} and Cheng \etal\cite{cheng2020learnedimagecompressiondiscretized}, particularly at lower bitrates.

% Adversarial examples have emerged as a significant concern in the field of machine learning, particularly affecting the robustness and security of deep learning models. These examples are inputs intentionally crafted to deceive models into making incorrect predictions. The phenomenon was first highlighted by Szegedy \etal \cite{szegedy2014intriguingpropertiesneuralnetworks}, who demonstrated that adding subtle, imperceptible perturbations to images could lead neural networks to misclassify them with high confidence.

% Kurakin \etal \cite{kurakin2017adversarialexamplesphysicalworld} extended the study of adversarial attacks to the physical world, demonstrating that printed images with adversarial perturbations could mislead classifiers even when captured through a camera. This work emphasized the practical implications of adversarial attacks beyond digital environments.

% In response to these challenges, various defense mechanisms have been proposed.
% Madry \etal \cite{madry2019deeplearningmodelsresistant} advocated for adversarial training, a process in which models are trained on adversarial examples to enhance their robustness. Papernot \etal \cite{papernot2016distillationdefenseadversarialperturbations} proposed defensive distillation, using distillation \cite{hinton2015distillingknowledgeneuralnetwork}, a technique designed to compress an ensemble of models into one smaller model, to create a model which is more robust to adversarial attacks. Another approach is to perform additional preprocessing steps to remove adversarial perturbations from an input before the classification step, which can be done by image compression\cite{dziugaite2016studyeffectjpgcompression}. 



% Despite these efforts, achieving comprehensive defense against adversarial attacks remains an open problem. Researchers continue to explore adaptive attack methods and corresponding defenses to better understand the underlying vulnerabilities of machine learning models and to develop more robust systems.
% \subsection{Image compression as adversarial defense}
% It has already been shown how JPEG compression can be used to increase the robustness of models against adversarial attacks. Dziugaite \etal \cite{dziugaite2016studyeffectjpgcompression} showed how JPEG can reverse the effect of small adversarial perturbations, even with a relatively high quality parameter of 75.0. To achieve this, an image, which may contain adversarial perturbations, is first compressed and then decompressed using JPEG compression. The small perturbations introduced by an adversarial attack are lost in this compression and decompression step.

% However, Shin \etal \cite{shin2017jpeg} shows how the effectiveness of the defensive property of JPEG can be reduced by using a differentiable approximation of the JPEG algorithm. They then propagate the gradient information through JPEG and the model when performing the adversarial attack. The adversarial perturbations created in this fashion persist through a JPEG compression and decompression step.

% \subsection{Learned lossy image compression}
% Learned lossy image compression is a technique that leverages machine learning to achieve efficient image compression. While traditional image compression algorithms like JPEG struggle to maintain high visual quality at very low bitrates, using learned compressions can lead to much clearer images at low bitrates \cite{agustsson2019generativeadversarialnetworksextreme}. This in turn leads to more information loss, which could be beneficial for an adversarial defense.

% HiFiC\cite{mentzer2020highfidelitygenerativeimagecompression} is a learned compression method that focuses on visually pleasing reconstructions, keeping information more important to human perception. The model uses an architecture based on Generative Adversarial Networks (GAN). The model was evaluated by a user study that showed that the resulting reconstructions were preferred to other methods even when using 2 times less bites per pixel.



% ELIC\cite{he2022elicefficientlearnedimage} which stands for Efficient Learned Image Compression with Unevenly Grouped Space-Channel Contextual Adaptive Coding, is a  model designed to optimize both the speed and efficiency of image compression.



==> sec/3_experiments.tex <==
\section{Methods}
\label{sec:methods}

The objective of our experiments was to evaluate the effectiveness of image compression as a defense mechanism against adversarial attacks. Additionally, we investigated the impact of varying compression quality levels and examined the effects of applying multiple compression steps sequentially.

We implemented our defenses as an additional preprocessing step applied to the (perturbed) image before it was fed into the classifier. Since lossy image compression inherently removes certain details, it is expected to eliminate some of the adversarial perturbations, thereby reducing the effectiveness of the attack. We then generated adversarial perturbations for the dataset and assessed the classifier’s accuracy on the perturbed images, comparing it to the baseline accuracy before the attack.

% The focus of our experiments was on assessing the strength of image compression as a defense against adversarial attacks. Additionally, we tested different qualities for the compressions used, and we conducted an experiment with multiple compressions in sequence.

% We defined our defenses as an additional step of preprocessing, which was computed for the (perturbed) image before feeding it to the classifier. Since we use lossy image compression, some parts of the introduced adversarial perturbations should be lost, thus negating the effect of the adversarial attack. We then computed adversarial perturbations for the dataset and evaluated the accuracy of the classifier on the newly generated images including the adversarial perturbation compared to the baseline accuracy before the attack. 

\subsection{Defenses}

The compression methods used as defenses were JPEG, HiFiC, and ELIC. JPEG was selected because it is one of the most widely used compression algorithms and has been previously explored as a defense mechanism against adversarial attacks \cite{dziugaite2016studyeffectjpgcompression, shin2017jpeg}. Thus, JPEG serves as a baseline for comparison with the other compression techniques. To implement JPEG compression and decompression, we used the differentiable approximation provided by Kornia \cite{eriba2019kornia}.

ELIC and HiFiC are both learned compression methods that utilize different architectures to achieve high image quality at low bitrates. PyTorch implementations and checkpoints with pretrained weights are publicly available for both methods\footnote{ELIC: \url{https://github.com/VincentChandelier/ELiC-ReImplemetation}} \footnote{HiFiC: \url{https://github.com/Justin-Tan/high-fidelity-generative-compression}}.

For HiFiC and ELIC, we employed differentiable forward functions. The use of differentiable defenses allowed gradient information to propagate through the entire pipeline (including both the model and the defense mechanism). This is expected to reduce the effectiveness of the defense, as it enables the adversarial attack to adapt its perturbations to persist through the compression process. To account for this, we conducted an additional set of experiments using this stronger adaptive attack. In tables throughout this paper, this is annotated with through being true.

% The compressions used as defenses were JPEG, HiFiC and ELIC. JPEG was used since it is one of the most commonly used compression algorithms and there has been prior work using JPEG as a defense against adversarial attacks \cite{dziugaite2016studyeffectjpgcompression}\cite{shin2017jpeg}. Therefore, JPEG provides a baseline to compare with the other compressions used. We used a differentiable approximation provided by Kornia\cite{eriba2019kornia} to compute the JPEG compression and decompression.

% ELIC and HiFiC are both learned compressions and use different architectures to achieve high image quality for low bitrates. For both a PyTorch implementation and pretrained weights are available \footnote{ElIC: \url{https://github.com/VincentChandelier/ELiC-ReImplemetation}} \footnote{HiFiC: \url{https://github.com/Justin-Tan/high-fidelity-generative-compression}}.

% For HiFiC and ELIC the differentiable forward functions were used. Using differentiable defenses enabled us to propagate the gradient information through the whole pipeline (model and defense) which should decrease the effectiveness of the defense, as the attack can adapt the introduced perturbations to persist through the compression. For all experiments, a version using this stronger attack was also conducted. 
\subsection{Adversarial attacks}

To compute adversarial images, we used the following methods:
\begin{itemize}
    \item Fast gradient sign method (FGSM)\cite{goodfellow2014explaining}
    \item Iterative FGSM (iFGSM) also called basic iterative method\cite{kurakin2017adversarialexamplesphysicalworld}
    \item Projected gradient descent (PGD)\cite{madry2019deeplearningmodelsresistant}
    \item Carlini-Wagner attack (CW)\cite{carlini2017evaluatingrobustnessneuralnetworks}
    \item DeepFool attack (DeepFool)\cite{moosavidezfooli2016deepfoolsimpleaccuratemethod}
\end{itemize}
For FGSM, iFGSM and PGD we use different $l_\infty$ norm values (epsilon) to modulate the attack strength, for CW and DeepFool we computed the accuracy for perturbations below a certain $l_2$ norm value. For iFGSM and PGD we used 10 iterations. For all attacks, the torchattacks\cite{kim2020torchattacks} implementation was used. For a full list of hyperparameters see supplementary table \ref{tab:hyperparams}.

\subsection{Models and datasets}
Two different base models were used in the experiments: one based on a ResNet50 architecture, ResNet50 \cite{he2015deepresiduallearningimage}, and a Vision Transformer (ViT), specifically ViT-B/16. Both models were sourced from PyTorch \cite{paszke2019pytorchimperativestylehighperformance} and initialized with pretrained ImageNet weights.

For our experiments, we used the validation split of Imagenette, a subset of ImageNet \cite{deng2009imagenet} containing 10 easily classified classes. In later experiments, the full ImageNet test split was utilized.

% Two different base models were used for the experiments,one based on a ResNet architecture, ResNet50\cite{he2015deepresiduallearningimage}, and a vision transformer (ViT), ViT\_b\_16 . Both models were provided by pytorch\cite{paszke2019pytorchimperativestylehighperformance} and the pretrained ImageNet weights were used. The validation split of Imagenette, a subset of ImageNet\cite{deng2009imagenet} with 10 easily classified classes, was used for our experiments; for later experiments the whole ImageNet test split was used. 

\subsection{Compression strength}

To determine the appropriate compression quality for our experiments, we conducted an additional series of tests for each compression method, comparing different levels to identify an optimal quality setting. Beyond defensive strength, our choice of compression was also influenced by several factors: the impact of the defense on accuracy in the absence of an attack, comparability between different compression methods and related work, and the availability of pretrained weights for learned compression models. Training these models from scratch was beyond the scope of this study.

The parameters influencing compression strength for the different methods were as follows:
\begin{itemize}
    \item \textbf{JPEG:} The quality parameter $q$ ranges from $0$ to $100$ and controls the quantization strength of the algorithm, with lower values corresponding to greater compression. We compared values $q \in \{5.0,10.0,15.0,25.0,35.0,50.0,75.0,95.0\}$. Typically, values greater than 70 are considered high quality, while values below 30 result in low-quality images that may appear pixelated and blurry.
    \item \textbf{HiFiC:} Three different sets of pretrained weights were available for HiFiC: $\textbf{HiFiC}^{\textbf{low}}$, $\textbf{HiFiC}^{\textbf{med}}$ and $\textbf{HiFiC}^{\textbf{hi}}$, which were trained to achieve target bitrates per pixel (BPP) of 0.14, 0.3, and 0.45, respectively.
    \item\textbf{ELIC:} Six different checkpoints were available for ELIC: [0004, 0008, 0016, 0032, 0150, 0450]. These correspond to different values of $\lambda$, the rate-controlling parameter, which determines the trade-off between estimated bitrate and image reconstruction distortion (for more details, see \cite{he2022elicefficientlearnedimage}).
\end{itemize}

Additionally, we computed BPP values for images from the ImageNet dataset, resized to $224\times224$ pixels, across different compression methods. This allowed for a direct comparison of size reduction between compression techniques.

\begin{table}[H]
    \centering
    \begin{tabular}{|c|c|}
    \hline
         \multicolumn{2}{|c|}{JPEG} \\
    \hline
    
    Quality & BPP \\
    
    \hline
         $q = 5.0$& 0.35\\
         \hline
         $q = 10.0$& 0.48\\
         \hline
         $q = 15.0$& 0.59\\
         \hline
         $q = 25.0$& 0.78\\
         \hline
         $q = 35.0$& 0.94\\
         \hline
         $q = 50.0$& 1.14\\
         \hline
         $q = 75.0$& 1.65\\
         \hline
         $q = 95.0$& 3.80\\
         \hline
    \end{tabular}
    \begin{tabular}{|c|c|}
    \hline
         \multicolumn{2}{|c|}{ELIC} \\
    \hline
    Weights & BPP\\
    
         \hline
         $0004$& 0.06\\
         \hline
         $0008$& 0.09\\
         \hline
         $0016$& 0.14\\
         \hline
         $0032$& 0.19\\
         \hline
         $0150$& 0.42\\
         \hline
         $0450$& 0.69\\
         \hline
         \multicolumn{2}{c}{}\\
         \multicolumn{2}{c}{}
         \vspace{1pt}

         
    \end{tabular}
    \begin{tabular}{|c|c|}
    \hline
         \multicolumn{2}{|c|}{HiFiC} \\
    \hline
    Weights & BPP\\
    
         \hline
         low& 0.15\\
         \hline
         med& 0.43\\
         \hline
         hi& 0.46\\
         \hline
         \multicolumn{2}{c}{}\\
         \multicolumn{2}{c}{}\\
         \multicolumn{2}{c}{}\\
         \multicolumn{2}{c}{}\\
         \multicolumn{2}{c}{}
         \vspace{2pt}

         
    \end{tabular}
    \caption{Bits per pixel for the different compressions and strengths used. Computed on 100 random images from ImageNet, sized down to $224\times224$}
    \label{tab:bpp}
\end{table}

\subsection{Sequential compression}
We also conducted experiments on the effectiveness of compressing and decompressing an image multiple times in sequence as a defense. For these experiments, we always propagated the gradient through the defense to achieve a stronger attack. The experiments were conducted on the Imagenette and on ImageNet. For ImageNet, we used 1000 randomly sampled images to reduce computation time.
\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.12\linewidth]{data/elic_1.png.png}
    \includegraphics[width=0.12\linewidth]{data/eliclow.png}
    \includegraphics[width=0.12\linewidth]{data/hific_1.png}
    \includegraphics[width=0.12\linewidth]{data/hific_med.png}
    \includegraphics[width=0.12\linewidth]{data/jpeg1.png}
    \includegraphics[width=0.12\linewidth]{data/elic_1adv.png.png}
    \caption{Images after they were compressed/decompressed multiple times. From left to right: ELIC:0016, ELIC:0004, HiFiC:low, HiFiC:med, JPEG:25.0, original image}
    \label{fig:images}
\end{figure*}
% To decide on the compression quality to use for our experiments, we concluded an additional series of experiments for each compression, comparing different levels to find an optimal quality. Beyond the defensive strength, our decision  on which compression to use was also influenced by the impact the defense had on the accuracy without an attack, comparability between the different compression methods used and to related work, and the availability of weights for the learned compressions. It was beyond the scope of this project to train these models from scratch. The parameters which impact compression strengths for the different compressions where:
% \begin{itemize}
%     \item JPEG. The quality parameter q is in the range $[0,100]$ and controls the quantization strength of the algorithm. Smaller values equate to greater compression. We compare  values $q \in \{5.0,10.0,15.0,25.0,35.0,50.0,75.0,95.0$\}. Values $>70.0$ are usually considered high quality, values $<30.0$ are low quality and can lead to pixelated and blurry images.
%     \item HiFiC. For HiFiC there were three different sets of pretrainded weights available $\textbf{HiFiC}^{\textbf{low}}$, $\textbf{HiFiC}^{\textbf{med}}$ and $\textbf{HiFiC}^{\textbf{hi}}$, which were trained to achieve a target bitrate per pixel(BPP) of 0.14,0.3 and 0.45 respectively.
%     \item ElIC. There were 6 different checkpoints available for ELIC: [0004,0008,0016,0032,0150,0450]. These checkpoints correspond to different values of  $\lambda$, the rate controlling parameter, which controls the ratio between the estimated bitrate and image reconstruction distortion (for more detail see \cite{he2022elicefficientlearnedimage}), used when training the model.
% \end{itemize}
% We also computed the BPP values on images from the ImageNet dataset, resized to the 224 x 224 pixels for the different compressions. This enabled us to compare qualities between compression methods.




==> sec/4_results.tex <==
\section{Results}
\label{sec:results}
The main results can be found in figures \ref{fig:l_inf} and \ref{fig:l_2}, the corresponding values in supplementary tables \ref{tab:linf_attacks_full} and \ref{tab:l2_attacks_full}.

\subsection{Baseline results}
  Both of the used models achieved a very high accuracy on Imagenette, $\approx 0.998$ for ResNet50 and $\approx 0.999$ for the ViT, as well as a strong resilience against the FGSM attack even without a defense, with both models still achieving accuracies $>0.8$ at an attack strength of epsilon $\frac{8}{255}$. For iFGSM and PGD the accuracy dropped to $<0.05$ for ResNet50 and $<0.01$ for the ViT at this level of attack strength. These baseline experiments also indicate a difference in robustness between the two models used, as the accuracy of the ViT is lower for all baseline experiments.
 
 \subsection{Defense results}
 \begin{figure}
     \centering
     \includegraphics[width=1.0\linewidth]{data//graphs/l_inf-6.pdf}
     \caption{Results of the FGSM, iFGSM and PGD attacks on the Imagenette dataset. Dashed lines show the results for the stronger attack, where the gradient was propagated through the defense. Epsilon values are shown in $\frac{x}{255}$}
     \label{fig:l_inf}
 \end{figure}
 \begin{figure}
     \centering
     \includegraphics[width=1.0\linewidth]{data//graphs/l_2-3.pdf}
     \caption{Results of the Carlini-Wagner and DeepFool attacks on the Imagenette dataset. Dashed lines show the results for the stronger attack, where the gradient was propagated through the defense. Epsilon shows the maximal $L_2$ norm of the perturbations.}
     \label{fig:l_2}
 \end{figure}



\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
         &Defense& Through & 0 & $\frac{4}{255}$ & $\frac{8}{255}$ & $\frac{12}{255}$  \\ \hline
         \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{ResNet50}}}  &  None  &  \cellcolor{lightgray}False &  \cellcolor{lightgray}100 &  \cellcolor{lightgray}6 &  \cellcolor{lightgray}4 &  \cellcolor{lightgray} 2 \\  \cline{2-7}
   &  \multirow{2}{*}{jpeg}  &  \cellcolor{lightblue}False &  \cellcolor{lightblue}100 &  \cellcolor{lightblue}99 &  \cellcolor{lightblue}98 &  \cellcolor{lightblue} 97 \\  \cline{3-7}
   &     &  \cellcolor{darkblue}True &  \cellcolor{darkblue}100 &  \cellcolor{darkblue}28 &  \cellcolor{darkblue}21 &  \cellcolor{darkblue} 17 \\  \cline{2-7}
   &  \multirow{2}{*}{ELIC}  &  \cellcolor{lightred}False &  \cellcolor{lightred}98 &  \cellcolor{lightred}98 &  \cellcolor{lightred}98 &  \cellcolor{lightred} 98 \\  \cline{3-7}
   &     &  \cellcolor{darkred}True &  \cellcolor{darkred}98 &  \cellcolor{darkred}54 &  \cellcolor{darkred}28 &  \cellcolor{darkred} 18 \\  \cline{2-7}
   &  \multirow{2}{*}{HiFiC}  &  \cellcolor{lightgreen}False &  \cellcolor{lightgreen}98 &  \cellcolor{lightgreen}97 &  \cellcolor{lightgreen}96 &  \cellcolor{lightgreen} 96 \\  \cline{3-7}
   &     &  \cellcolor{darkgreen}True &  \cellcolor{darkgreen}98 &  \cellcolor{darkgreen}38 &  \cellcolor{darkgreen}20 &  \cellcolor{darkgreen} 12 \\  \cline{1-7}
\parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{ViT}}}  &  None  &  \cellcolor{lightgray}False &  \cellcolor{lightgray}100 &  \cellcolor{lightgray}4 &  \cellcolor{lightgray}1 &  \cellcolor{lightgray} 0 \\  \cline{2-7}
   &  \multirow{2}{*}{jpeg}  &  \cellcolor{lightblue}False &  \cellcolor{lightblue}100 &  \cellcolor{lightblue}90 &  \cellcolor{lightblue}56 &  \cellcolor{lightblue} 26 \\  \cline{3-7}
   &     &  \cellcolor{darkblue}True &  \cellcolor{darkblue}100 &  \cellcolor{darkblue}11 &  \cellcolor{darkblue}4 &  \cellcolor{darkblue} 2 \\  \cline{2-7}
   &  \multirow{2}{*}{ELIC}  &  \cellcolor{lightred}False &  \cellcolor{lightred}99 &  \cellcolor{lightred}98 &  \cellcolor{lightred}97 &  \cellcolor{lightred} 95 \\  \cline{3-7}
   &     &  \cellcolor{darkred}True &  \cellcolor{darkred}99 &  \cellcolor{darkred}50 &  \cellcolor{darkred}20 &  \cellcolor{darkred} 9 \\  \cline{2-7}
   &  \multirow{2}{*}{HiFiC}  &  \cellcolor{lightgreen}False &  \cellcolor{lightgreen}100 &  \cellcolor{lightgreen}99 &  \cellcolor{lightgreen}98 &  \cellcolor{lightgreen} 97 \\  \cline{3-7}
   &     &  \cellcolor{darkgreen}True &  \cellcolor{darkgreen}100 &  \cellcolor{darkgreen}26 &  \cellcolor{darkgreen}8 &  \cellcolor{darkgreen} 4 \\  \hline


    \end{tabular}
    \caption{Accuracies(in \%) of our defenses for iFGSM with different epsilon values on the Imagentte dataset, rounded to two digits.}
    \label{tab:linf_small}
\end{table}

 \begin{figure}
     \centering
     \includegraphics[width=1.0\linewidth]{data//graphs/l_inf_1000.pdf}
     \caption{Results of the FGSM, iFGSM and PGD attacks on 1000 images from the ImageNet dataset. Dashed lines show the results for the stronger attack, where the gradient was propagated through the defense. Epsilon values are shown in $\frac{x}{255}$}
     \label{fig:l_inf_1000}
 \end{figure}


All 3 defense methods showed promising results, showing almost no change in accuracy after all attacks when using the ResNet50 model (see figures \ref{fig:l_inf} and \ref{fig:l_2}). Using the ViT, iFGSM and PGD lead to a drop in accuracy at epsilon $\frac{4}{255}$ for JPEG, but still achieve a much higher accuracy than the baseline. The learned compression algorithms show better performance for the ViT, with both ELIC and HiFiC achieving an accuracy comparable to before the attack even for high values of epsilon.

Adversarial images crafted with the Carlini-Wagner and DeepFool attacks were less difficult to defend against. This could possibly be attributed to the fact that these attacks find minimal perturbations, compared to the other 3 attacks used, which find perturbations within the given bounds, which are not necessarily minimal. There are also more hyperparameters, which need tuning for an optimal attack, and a longer runtime. These factors lead us to focus less on these attacks and not conduct additional experiments with Carlini-Wagner and DeepFool.

Attacking the entire pipeline drastically weakens the effect of all three defenses. There is still improvement over no defense at all, but the accuracy is not comparable to the experiments where the gradient information was not propagated through the defenses.

These Results indicate three major things:
\begin{itemize}
    \item The ViT used is less robust against adversarial attack.
    \item The learned compressions used perform better for the ViT.
    \item The effectiveness of a compression based defense can be greatly diminished by creating adversarial images which include gradient information propagated through the defense in their computation.
\end{itemize}
\subsubsection{ImageNet results}
After analyzing these results we decided to repeat some experiments on 1000 random images taken from the ImageNet dataset, to see how the defenses perform in this harder task, with 1000 possible classes instead of 10 and a much lower baseline accuracy (both models achieve an accuracy of about 0.8 on ImageNet). The results of these experiments can be found in figure \ref{fig:l_inf_1000}. In this experimental setup, all defenses show a larger accuracy decrease without an attack. This decrease is larger for ResNet50 than for the ViT. There is also a more noticeable decrease as the epsilon constraint of the attack gets larger for all attacks. On Imagenette the accuracy was almost constant for effective defenses. But generally the results on ImageNet show the same trends already discussed in the previous section.

\subsection{Computational overhead}
We also computed the time it takes the model during inference to show the feasibility of these defenses in practice. Note that this is not a thorough investigation of runtimes. For this test, we used an Nvidia RTX3090 and ResNet50. We did not include the time the models need to initialize. Without a defense it took 20.8 seconds to classify the 3925 images in the Imagenette dataset, or 0.005 seconds per image. With JPEG as a defense, it took 31.3 seconds, or 0.008 seconds per image. Using ELIC it took  54.5 seconds, 0.014 seconds per image and using HiFiC it took 54.8, or 0.014 per image. Even when compressing and decompressing the images 5 times in sequence, this only increased to 130 seconds for HiFiC, 136 seconds for ELIC. 50 times JPEG in sequence took 111 seconds. This is a small increase and shows all these methods are feasible to implement in a real world setting.






\subsection{Quality ablation}
In this section, we show a comparison between different compression strengths for all the compressions used as defenses. Complete tables can be found in the appendix, see tables \ref{tab:abl_jpeg} \ref{tab:abl_hific} \ref{tab:alb_elic}.

\begin{figure}[H]
    \centering
    \includegraphics[width=1.0\linewidth]{data//graphs/jpeg_abl-2.pdf}
    \caption{Accuracies for different qualities of JPEG compression, iFGSM attack, dashed lines show the results when gradient information was available to the attack.Top: ResNet50, bottom: ViT }
    \label{fig:abl_jpeg}
\end{figure}
\subsubsection{JPEG}
Figure \ref{fig:abl_jpeg} shows the accuracy for different JPEG qualities when attacked with iFGSM. For ResNet50, only the high quality levels (75.0,95.0) were vulnerable to a standard attack. When using the stronger attack which propagates the gradients through the defense, no quality level did achieve a high accuracy and therefore a successful defense. Accuracy levels 15.0 and 25.0 achieved the highest accuracy at $\approx 0.2$. In the ViT experiment, a larger spread of results can be observed, with lower quality levels performing better at high epsilon values. JPEG with a quality level of 5.0 showed a large decrease in accuracy without any attack. taking these observations into consideration, we decided to use a quality level of 25.0, as this achieves a good performance, does not degrade the baseline accuracy and has been used in previous work by Shin \etal \cite{shin2017jpeg}.


\subsubsection{HiFiC}
Figure \ref{fig:abl_hific} shows that all the different compression strengths worked well as a defense for ResNet50, but only HiFiC low achieved a high accuracy for the ViT, with the other two quality showing a decrease in accuracy for epsilon larger than $ \frac{4}{255}$. All levels were very vulnerable when the gradient was passed through the defense. Since the lowest quality only showed little decrease in baseline performance, we decided to use HiFiC low for the main experiments.
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{data/graphs/hific_abl-2.pdf}
    \caption{Accuracies for different qualities of HiFiC, iFGSM attack, dashed lines show the results when gradient information was available to the attack.Top: ResNet50, bottom: ViT }
    \label{fig:abl_hific}
\end{figure}
\subsubsection{ELIC}
Figure \ref{fig:abl_elic} shows the results for ELIC. The higher quality levels show decreased performance for high epsilon values. The lowest quality levels show a decreased accuracy without any attack. There is a larger difference between quality levels when the gradient is propagated through the defense compared to HiFiC. For the main experiment we decided to use ELIC 0016, as it achieved good accuracies without visibly decreasing the baseline performance, and because it is similar in BPP to HiFiC low. 
\begin{figure}[h]
    \centering
    \includegraphics[width=1.0\linewidth]{data//graphs/elic_abl.pdf}
    \caption{Accuracies for different qualities of ELIC, iFGSM attack, dashed lines show the results when gradient information was available to the attack.Top: ResNet50, bottom: ViT }
    \label{fig:abl_elic}
\end{figure}
\FloatBarrier

\subsection{Sequential defense}
\subsubsection{Imagenette}
For JPEG, we used quality level 25.0 for the results shown in figures \ref{fig:seq-jpeg_large} and \ref{fig:seq-jpeg_small}. For HiFiC and ELIC there is a tradeoff between a decrease in accuracy without an attack for low qualities and a decrease in effectiveness for high qualities. The baseline accuracy using HiFiC:low deteriorates quickly, making it unusable as a sequential defense, see figure \ref{fig:hific_seq_low}. ELIC:0016 also decreases the baseline accuracy, but much slower than HiFiC:low. This leads to a promising defense which reaches close to baseline accuracy with 7 sequential defense iterations, as can be seen in figure \ref{fig:elic_seq_low}.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data//graphs//seq/hific_seq_low.pdf}
    \caption{HiFiC:low used as a sequential defense. Computed using iFGSM, ResNet50
and Imagenette.}
    \label{fig:hific_seq_low}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data//graphs//seq/elic_seq_low.pdf}
    \caption{ELIC:0016 used as a sequential defense. Computed using iFGSM, ResNet50
and Imagenette.}
    \label{fig:elic_seq_low}
\end{figure}
The experiments indicate a clear trend, showing that running an image through a defense multiple times increases its effectiveness for all defenses. JPEG showed the fastest increase, achieving an accuracy of over 0.9 for epsilon $\frac{8}{255}$ after 5 iterations and converging towards the baseline. The decrease in baseline accuracy for JPEG is negligible even after 50 iterations. HiFiC and ELIC also show an increased accuracy for each additional sequential iteration, achieving accuracies of about 0.4 with 7 iterations. Because of the large amount of gradient information, we were unable to compute results for more than 7 iterations of ELIC or HiFiC.

Figure \ref{fig:images} shows how the image quality deteriorates when compressing and decompressing multiple times in sequence. Both of the learned compressions show a stark difference to the original image. ELIC introduces black/red artifacts which take up parts of the image. The lowest quality of HiFiC leads to a much brighter image, which lost most of the color information. JPEG  performed best, while it also introduces artifacts and blurs the image a lot, the image still looks similar after multiple passes through the compression.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/jpeg_seq_large.pdf}
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/imagnette_seq.pdf}
    \caption{Accuracy of the sequential defense using multiple iterations. Top: JPEG defense, bottom comparison between JPEG, HiFiC, ELIC for epsilon $\frac{8}{255}$. Computed using iFGSM,  ResNet50 and Imagenette.}
    \label{fig:seq-jpeg_large}
\end{figure}
\subsubsection{ImageNet}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/jpeg_seq_imagenet_rn_qs.pdf}
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/jpeg_seq_imagenet_ViT_qs.pdf}
    \caption{Accuracy of the sequential JPEG defense after an iFGSM attack for different quality levels on 1000 images from ImageNet. Top: ViT, bottom ResNet50.}
    \label{fig:seq_jpeg_inet}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/jpeg_seq_imagenet_rn_qs_base.pdf}
    \caption{Baseline accuracy with no attack for different quality levels on 1000 images from ImageNet using ResNet50.}
    \label{fig:seq-jpeg_inetbase}
\end{figure}

Experiments on sequential defense using JPEG on the harder ImageNet dataset showed similar results, as can be seen in figure \ref{fig:seq_jpeg_inet} for different quality levels. The achieved accuracy is lower compared to the previous experiments. This can in part be attributed to a larger decrease in baseline accuracy. Lower quality levels show a decrease in accuracy on images without an attack. This decrease seems to depend mostly on the quality parameter, as the accuracy stays relatively constant with multiple iterations.

The jaggedness of the lines compared to the Imagenette results could come from the random sampling used.
But even taking the lower baselines into consideration, no quality seems to converge towards the baseline with 10 sequential passes. This indicates a deeper sequential defense is needed for this harder task.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{data/graphs/seq/jpeg_seq_imagenet_deep.pdf}
    \caption{Deeper version of the defense for JPEG q=10.0 and q=95.0, dashed line shows the baseline accuracy.Computed using iFGSM with epsilon=$\frac{8}{255}$, ResNet50
and Imagenette. }
    \label{fig:seq_jpeg_deep}
\end{figure}

An experiment with a deeper sequential JPEG defense, see figure \ref{fig:seq_jpeg_deep}, shows how this is the case, as quality 10.0 seems to converge. For quality 95.0 the accuracy still improves even at 50 iterations. The jaggedness of the baseline for low iterations is due to different subsets of ImageNet being used. This was changed later in the experiment for more consistent results.
\FloatBarrier






==> sec/5_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we analyze the efficiency of image compressions as adversarial defenses. We show learned compressions have advantages over conventional compression algorithms, as they do not significantly decrease the baseline accuracy of an image classification model even at low BPP. We also show the weaknesses of such defenses in a white-box setting, as a gradient can either be directly computed or approximated, which then decreases the defense's effectiveness. We also show how sequentially running an image through such a defense can provide additional robustness.

There are however also some limitations, as we limit our experiments to gradient based attacks constrained on the $L_\infty$ or $L_2$ norm. In real world settings, there are more possible ways to attack a model (Engstrom \etal \cite{engstrom2019exploringlandscapespatialrobustness}, Gilmer \etal \cite{gilmer2018motivatingrulesgameadversarial}). We also did not compare to gradient free attacks\cite{uesato2018adversarialriskdangersevaluating}. Further work could include results for these defenses in a setting which takes these additional threats into account and combine image compression with other defensive measures to create more robust deep learning models.




